Final Architecture Specification of security, privacy, and incentive mechanisms

In this document, we define the NADA security architecture based on refined use case scenarios, a derived high level model and security analysis. For the architecure design and verification we are applying the well known STRIDE model.

==> dfd.tex <==

\LTXtable{\ltablewidth}{dfd_entities}
\LTXtable{\ltablewidth}{dfd_threats}
\LTXtable{\ltablewidth}{measures}
\LTXtable{\ltablewidth}{dfd_threat_measures}
\LTXtable{\ltablewidth}{dfd_threat_measures_long}
